The Power of Input: Benchmarking Zero-Shot Sim-To-Real Transfer of Reinforcement Learning Control Policies for Quadrotor Control

In the last decade, data-driven approaches have become popular choices for quadrotor control, thanks to their ability to facilitate the adaptation to unknown or uncertain flight conditions. Among the different data-driven paradigms, Deep Reinforcement Learning (DRL) is currently one of the most explored. However, the design of DRL agents for Micro Aerial Vehicles (MAVs) remains an open challenge. While some works have studied the output configuration of these agents (i.e., what kind of control to compute), there is no general consensus on the type of input data these approaches should employ. Multiple works simply provide the DRL agent with full state information, without questioning if this might be redundant and unnecessarily complicate the learning process, or pose superfluous constraints on the availability of such information in real platforms. In this work, we provide an in-depth benchmark analysis of different configurations of the observation space. We optimize multiple DRL agents in simulated environments with different input choices and study their robustness and their sim-to-real transfer capabilities with zero-shot adaptation. We believe that the outcomes and discussions presented in this work supported by extensive experimental results could be an important milestone in guiding future research on the development of DRL agents for aerial robot tasks.

==> figures/learning.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/train500smallok.png}
    \caption{\changes{Learning curves of the DRL controllers: we report the cumulative reward reached by each agent during the training phase.}}
    \vspace{-1em}
    \label{fig:learning} 
\end{figure}

==> figures/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/overview.png}
    \caption{Overview of the benchmark study: we investigate the impact of different input configurations on the ability of a Deep Reinforcement Learning policy to fly a real drone.}
    \vspace{-1.5em}
    \label{fig:overview} 
\end{figure*}

==> tables/sim_tab_angular_metric.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Mean of the accumulated angular velocities in rad/s across different scenarios.}
\resizebox{\textwidth}{!}{
\label{tab:simresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{\shortstack{Observation\\Space\\Configuration}} & \multicolumn{16}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-17}
& \multicolumn{4}{c|}{Hovering} & \multicolumn{4}{c|}{Planar Ellipse} & \multicolumn{4}{c|}{Planar Eight-Shape} & \multicolumn{4}{c|}{3D Eight-Shape}\\
\cline{2-17}
& $A_{\omega x}$ & $A_{\omega y}$ & $A_{\omega z}$ & $A_{c}$ & $A_{\omega x}$ & $A_{\omega y}$ & $A_{\omega z}$ & $A_{c}$ & $A_{\omega x}$ & $A_{\omega y}$ & $A_{\omega z}$ & $A_{c}$ & $A_{\omega x}$ & $A_{\omega y}$ & $A_{\omega z}$ & $A_{c}$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  0.07$ & $  0.04$ & $  0.04 $ & $ \cellcolor{green!30} 0.05$ & $  0.10$ & $  0.10 $ & $ 0.09 $ & $ \cellcolor{green!30} 0.10$ & $ 0.08$ & $  0.07 $ & $  0.07 $ & $ \cellcolor{green!30} 0.07$ & $  0.09$ & $  0.07 $ & $  0.06 $ & $ \cellcolor{green!30} 0.07$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $  0.06 $ & $  0.08 $ & $  0.04$ & $ \cellcolor{yellow!30} 0.06$ & $  0.13 $ & $  0.10 $ & $  0.09$ & $ \cellcolor{yellow!30} 0.11$ & $  0.08 $ & $  0.10 $ & $ 0.05 $ & $ \cellcolor{yellow!30} 0.08$ & $  0.08$ & $ 0.09 $ & $  0.05$ & $ \cellcolor{green!30} 0.07$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  0.03 $ & $  0.04 $ & $  0.06 $ & $ \cellcolor{green!30} 0.04$ & $  0.12 $ & $  0.12 $ & $  0.25 $ & $ \cellcolor{red!30} 0.17$ & $  0.06 $ & $  0.07 $ & $  0.15 $ & $ \cellcolor{red!30} 0.09$ & $  0.07 $ & $  0.09$ & $  0.17 $ & $ \cellcolor{red!30} 0.11$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  0.06 $ & $ 0.07 $ & $  0.07 $ & $ \cellcolor{yellow!30} 0.06$ & $  0.13 $ & $  0.11 $ & $ 0.21$ & $ \cellcolor{red!30} 0.15$ & $  0.08 $ & $0.09$ & $  0.12 $ & $ \cellcolor{red!30} 0.10$ & $  0.08 $ & $  0.10 $ & $ 0.14 $ & $ \cellcolor{red!30} 0.10$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  0.06 $ & $  0.05 $ & $  0.02 $ & $ \cellcolor{green!30} 0.05$ & $  0.14 $ & $  0.11 $& $  0.07 $& $ \cellcolor{green!30} 0.10$& $  0.08 $& $  0.08 $& $  0.04 $& $ \cellcolor{green!30} 0.07$& $  0.09 $& $  0.09 $& $  0.05 $& $ \cellcolor{yellow!30} 0.08$\\
\hline
$\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$ & $ 0.10$ & $  0.06$ & $  0.05$ & $ \cellcolor{red!30} 0.07$ & $  0.13 $ & $  0.09 $& $  0.08 $& $ \cellcolor{green!30} 0.10$& $  0.11 $& $  0.08 $& $  0.06 $& $ \cellcolor{yellow!30} 0.08$& $  0.11 $& $  0.08 $& $  0.06 $& $ \cellcolor{yellow!30} 0.08$\\
\hline
\end{tabular}}
\vspace{-1.0em}
\end{table*}

==> tables/sim_tab_res.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Simulation results: positional tracking error in centimeters across different scenarios.}
\resizebox{\textwidth}{!}{
\label{tab:simresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{\shortstack{Observation\\Space\\Configuration}} & \multicolumn{16}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-17}
& \multicolumn{4}{c|}{Hovering} & \multicolumn{4}{c|}{Planar Ellipse} & \multicolumn{4}{c|}{Planar Eight-Shape} & \multicolumn{4}{c|}{3D Eight-Shape}\\
\cline{2-17}
& $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  \textbf{0.2}$ & $  0.3$ & $  1.3 $ & $ \cellcolor{red!30} 0.6$ & $  4.9$ & $  5.4 $ & $ 1.0 $ & $ \cellcolor{red!30} 3.8$ & $ 2.2$ & $  2.8 $ & $  1.3 $ & $ \cellcolor{red!30} 2.1$ & $  2.5$ & $  2.9 $ & $  1.3 $ & $ \cellcolor{red!30} 2.2$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $  0.3 $ & $  \textbf{0.2} $ & $  0.5$ & $ \cellcolor{green!30} \textbf{0.4}$ & $  1.0 $ & $  2.6 $ & $  1.1$ & $ \cellcolor{yellow!30} 1.5$ & $  1.3 $ & $  1.0 $ & $ 0.9 $ & $ \cellcolor{yellow!30} 1.1$ & $  \textbf{1.1}$ & $ 1.0 $ & $  1.0$ & $ \cellcolor{green!30} \textbf{1.0}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  0.5 $ & $  0.3 $ & $  0.7 $ & $ \cellcolor{red!30} 0.5$ & $  2.7 $ & $  \textbf{1.9} $ & $  3.3 $ & $ \cellcolor{red!30} 2.6$ & $  2.6 $ & $  1.1 $ & $  1.5 $ & $ \cellcolor{red!30} 1.7$ & $  2.9 $ & $  1.2$ & $  1.8 $ & $ \cellcolor{red!30} 2.0$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  0.3 $ & $ 0.6 $ & $  \textbf{0.4} $ & $ \cellcolor{yellow!30} 0.5$ & $  1.0 $ & $  2.0 $ & $ 1.3$ & $ \cellcolor{yellow!30} 1.5$ & $  \textbf{1.0} $ & $1.1$ & $  0.8 $ & $ \cellcolor{green!30} 1.0$ & $  \textbf{1.1} $ & $  1.2 $ & $ 1.4 $ & $ \cellcolor{yellow!30} 1.2$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  0.3 $ & $  0.3 $ & $  0.5 $ & $ \cellcolor{green!30} \textbf{0.4}$ & $  1.1 $ & $  2.0 $& $  \textbf{0.6} $& $ \cellcolor{green!30} \textbf{1.2}$& $  1.3 $& $  \textbf{0.8} $& $  \textbf{0.6} $& $ \cellcolor{green!30} \textbf{0.9}$& $  1.3 $& $  \textbf{0.8} $& $  \textbf{0.9} $& $ \cellcolor{green!30} \textbf{1.0}$\\
\hline
$\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$ & $ \textbf{0.2}$ & $  0.5$ & $  0.9$ & $ \cellcolor{yellow!30} 0.5$ & $  \textbf{0.9} $ & $  \textbf{1.9} $& $  1.2 $& $ \cellcolor{green!30} 1.3$& $  1.3 $& $  \textbf{0.8} $& $  1.0 $& $ \cellcolor{green!30} 1.0$& $  1.3 $& $  0.9 $& $  1.5 $& $ \cellcolor{yellow!30} 1.2$\\
\hline
\end{tabular}}
\vspace{-1.0em}
\end{table*}

==> tables/sim_tab_res_vel.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Simulation results: positional tracking error in centimeters of the experiments conducted at increased speed.}
\resizebox{\textwidth}{!}{
\label{tab:simvelresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{\shortstack{Observation\\Space\\Configuration}} & \multicolumn{12}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-13} & \multicolumn{4}{c|}{Planar Ellipse} & \multicolumn{4}{c|}{Planar Eight-Shape} & \multicolumn{4}{c|}{3D Eight-Shape}\\
\cline{2-13}
& $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  17.6$ & $  11.1$& $  4.2 $& $ \cellcolor{red!30} 11.0$& $  8.5 $& $  7.5 $& $  2.3 $& $ \cellcolor{red!30} 6.1$& $  10.1 $& $ 7.4$& $  5.7$& $ \cellcolor{red!30} 7.7$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $  \textbf{2.7} $ & $  11.4 $& $  2.3 $& $ \cellcolor{green!30} 5.5$& $ \textbf{3.3}$& $  2.6 $& $  1.5 $& $ \cellcolor{green!30} 2.5$& $  \textbf{2.8} $& $  2.8 $& $  \textbf{4.0}$& $ \cellcolor{green!30} \textbf{3.2}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  5.3 $ & $  15.8 $& $  9.4 $& $ \cellcolor{red!30} 10.2$& $  5.4 $& $  2.4 $& $  3.2$& $ \cellcolor{red!30} 3.7$& $  6.0$& $  2.7 $& $  6.2$& $ \cellcolor{red!30} 4.9$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  3.9 $ & $  10.6 $& $  4.3 $& $ \cellcolor{yellow!30} 6.3$& $  4.5 $& $  \textbf{1.9}$& $  2.3$& $ \cellcolor{yellow!30} 2.9$& $  5.2$& $  \textbf{1.9} $& $  5.5 $& $ \cellcolor{yellow!30} 4.2$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  7.2 $ & $  9.2 $& $  2.2 $& $ \cellcolor{yellow!30} 6.2$& $  4.2 $& $  2.1 $& $  \textbf{0.8} $& $ \cellcolor{green!30} \textbf{2.4}$& $  4.1 $& $  2.7 $& $  4.3 $& $ \cellcolor{green!30} 3.7$ \\
\hline
$\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$  & $  5.2 $ & $  \textbf{8.0} $& $  \textbf{1.8} $& $ \cellcolor{green!30} \textbf{5.0}$& $  5.9 $& $  2.4 $& $  2.3 $& $ \cellcolor{yellow!30} 3.6$& $  5.9 $& $  2.8 $& $  5.6 $& $ \cellcolor{yellow!30} 4.8$ \\
\hline
\end{tabular}}
\vspace{-1.0em}
\end{table*}

==> tables/tab_res.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Experimental results: positional tracking error in centimeters across different scenarios.}
\resizebox{\textwidth}{!}{
\label{tab:results}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{\shortstack{Observation\\Space\\Configuration}} & \multicolumn{16}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-17}
& \multicolumn{4}{c|}{Hovering} & \multicolumn{4}{c|}{Planar Ellipse} & \multicolumn{4}{c|}{Planar Eight-Shape} & \multicolumn{4}{c|}{3D Eight-Shape}\\
\cline{2-17}
& $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  5.0$ & $  6.9$ & $  \textbf{2.1} $ & $ \cellcolor{red!30} 4.6$ & $  7.9$ & $  6.6 $ & $ \textbf{2.7} $ & $ \cellcolor{red!30} 5.7$ & $ 9.8$ & $  7.1 $ & $  3.4 $ & $ \cellcolor{red!30} 6.8$ & $  9.6$ & $  8.5 $ & $  6.0 $ & $ \cellcolor{red!30} 8.1$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $  2.6 $ & $  \textbf{2.1} $ & $  3.3$ & $ \cellcolor{green!30} \textbf{2.7}$ & $  \textbf{2.3} $ & $  3.4 $ & $  3.2$ & $ \cellcolor{green!30} \textbf{3.0}$ & $  \textbf{2.7} $ & $  \textbf{2.8} $ & $ 4.1 $ & $ \cellcolor{green!30} \textbf{3.1}$ & $  \textbf{2.5}$ & $ 2.9 $ & $  6.2$ & $ \cellcolor{green!30} \textbf{3.9}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  4.7 $ & $  3.0 $ & $  3.2 $ & $ \cellcolor{red!30} 3.7$ & $  6.7 $ & $  4.2 $ & $  4.4 $ & $ \cellcolor{red!30} 5.1$ & $  9.5 $ & $  3.1 $ & $  \textbf{3.1} $ & $ \cellcolor{red!30} 5.2$ & $  8.0 $ & $  2.9$ & $  6.6 $ & $ \cellcolor{red!30} 5.8$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  2.5 $ & $ 2.7 $ & $  3.1 $ & $ \cellcolor{green!30} \textbf{2.7}$ & $  4.0 $ & $  \textbf{3.3} $ & $ 3.6$ & $ \cellcolor{green!30} 3.6$ & $  4.1 $ & $3.0 $ & $  3.6 $ & $ \cellcolor{green!30} 3.5$ & $  3.1 $ & $  \textbf{2.6} $ & $ \textbf{5.8} $ & $ \cellcolor{green!30} \textbf{3.9}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  \textbf{2.1} $ & $  3.2 $ & $  2.7 $ & $ \cellcolor{green!30} \textbf{2.7}$ & $  3.7 $ & $  5.0 $ & $  3.2$ & $ \cellcolor{yellow!30} 4.0$ & $  3.5$ & $  4.2 $  & $ 3.3 $ & $ \cellcolor{yellow!30} 3.6$ & $  4.2 $ & $  4.5 $ & $  \textbf{5.8} $ & $ \cellcolor{yellow!30} 4.8$\\
\hline
$\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$ & $ 2.2$ & $  3.7$ & $  3.1$ & $ \cellcolor{yellow!30} 3.0$ & $  3.2$ & $  4.7$ & $  3.0$ & $ \cellcolor{green!30} 3.6$ & $  3.3$ & $  4.2 $  & $  3.9 $ & $ \cellcolor{yellow!30} 3.8$ & $  3.5$ & $  4.3$ & $ 6.7$ & $ \cellcolor{yellow!30} 4.8$\\
\hline
\hline
PID Controller & $ 1.6$ & $  1.5$ & $  1.4$ & $ \cellcolor{green!30} 1.5$ & $  2.4$ & $  5.5$ & $  1.6$ & $ \cellcolor{green!30} 3.2$ & $  2.8$ & $  2.7 $  & $  1.5 $ & $ \cellcolor{green!30} 2.3$ & $  3.4$ & $  2.6$ & $ 8.7$ & $ \cellcolor{yellow!30} 4.9$\\
\hline
\end{tabular}}
\vspace{-1.0em}
\end{table*}

==> tables/tab_res_backup.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{\textcolor{red}{MIGLIORARE Experimental results. We report the mean over 3 runs of the x y z error RMSE and (peak) values.}}
\resizebox{\textwidth}{!}{
\label{tab:results}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{Input Type} & \multicolumn{16}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-17}
& \multicolumn{4}{c|}{Hovering Trajectory} & \multicolumn{4}{c|}{Planar Oval Trajectory} & \multicolumn{4}{c|}{Planar Eight Trajectory} & \multicolumn{4}{c|}{Spatial Eight Trajectory}\\
\cline{2-17}
& $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  5.0 \,(11.6)$ & $  6.9 \,(12.9)$ & $  \textbf{2.1} \,(\textbf{5.3})$ & $ \cellcolor{red!30} 4.6$ & $  7.9 \,(18.1)$ & $  6.6 \,(14.4)$ & $ \textbf{2.7} \,(\textbf{6.7})$ & $ \cellcolor{red!30} 5.7$ & $ 9.8 \,(21.2)$ & $  7.1 \,(13.6)$ & $  3.4 \,(8.4)$ & $ \cellcolor{red!30} 6.8$ & $  9.6 \,(19.3)$ & $  8.5 \,(17.4)$ & $  6.0 \,(11.7)$ & $ \cellcolor{red!30} 8.1$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $  2.6 \,(\textbf{5.8})$ & $  \textbf{2.1} \,(\textbf{6.3})$ & $  3.3 \,(8.6)$ & $ \cellcolor{green!30} \textbf{2.7}$ & $  \textbf{2.3} \,(\textbf{5.9})$ & $  3.4 \,(\textbf{8.4})$ & $  3.2 \,(8.6)$ & $ \cellcolor{green!30} \textbf{3.0}$ & $  \textbf{2.7} \,(\textbf{5.9})$ & $  \textbf{2.8} \,(\textbf{7.5})$ & $ 4.1 \,(10.4)$ & $ \cellcolor{green!30} \textbf{3.1}$ & $  \textbf{2.5} \,(\textbf{6.3})$ & $ 2.9 \,(9.5)$ & $  6.2 \,(13.5)$ & $ \cellcolor{green!30} \textbf{3.9}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  4.7 \,(10.4)$ & $  3.0 \,(6.8)$ & $  3.2 \,(7.8)$ & $ \cellcolor{red!30} 3.7$ & $  6.7 \,(17.7)$ & $  4.2 \,(12.4)$ & $  4.4 \,(10.0)$ & $ \cellcolor{red!30} 5.1$ & $  9.5 \,(18.9)$ & $  3.1 \,(8.6)$ & $  \textbf{3.1} \,(8.2)$ & $ \cellcolor{red!30} 5.2$ & $  8.0 \,(18.2)$ & $  2.9 \,(\textbf{7.5})$ & $  6.6 \,(16.0)$ & $ \cellcolor{red!30} 5.8$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  2.5 \,(6.5)$ & $ 2.7 \,(7.2)$ & $  3.1 \,(7.6)$ & $ \cellcolor{green!30} \textbf{2.7}$ & $  4.0 \,(11.8)$ & $  \textbf{3.3} \,(10.3)$ & $ 3.6 \,(8.3)$ & $ \cellcolor{green!30} 3.6$ & $  4.1 \,(11.5)$ & $3.0 \,(8.8)$ & $  3.6 \,(7.2)$ & $ \cellcolor{green!30} 3.5$ & $  3.1 \,(7.1)$ & $  \textbf{2.6} \,(7.9)$ & $ \textbf{5.8} \,(\textbf{13.2})$ & $ \cellcolor{green!30} \textbf{3.9}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  \textbf{2.1} \,(6.0)$ & $  3.2 \,(8.5)$ & $  2.7 \,(7.6)$ & $ \cellcolor{green!30} \textbf{2.7}$ & $  3.7 \,(8.6)$ & $  5.0 \,(11.9)$ & $  3.2 \,(8.5)$ & $ \cellcolor{yellow!30} 4.0$ & $  3.5 \,(9.6)$ & $  4.2 \,(10.0)$  & $ 3.3 \,(\textbf{7.7})$ & $ \cellcolor{yellow!30} 3.6$ & $  4.2 \,(10.1)$ & $  4.5 \,(11.1)$ & $  \textbf{5.8} \,(13.6)$ & $ \cellcolor{yellow!30} 4.8$\\
\hline
$\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$ & $ 2.2 \,(6.1)$ & $  3.7 \,(10.2)$ & $  3.1 \,(8.2)$ & $ \cellcolor{yellow!30} 3.0$ & $  3.2 \,(8.1)$ & $  4.7 \,(12.5)$ & $  3.0 \,(8.2)$ & $ \cellcolor{green!30} 3.6$ & $  3.3 \,(8.4)$ & $  4.2 \,(10.2)$  & $  3.9 \,(10.2)$ & $ \cellcolor{yellow!30} 3.8$ & $  3.5 \,(8.0)$ & $  4.3 \,(10.8)$ & $ 6.7 \,(15.2)$ & $ \cellcolor{yellow!30} 4.8$\\
\hline
\end{tabular}}
\vspace{-0.8em}
\end{table*}








% \begin{table*}[t]
% \renewcommand{\arraystretch}{1.3}
% \centering
% \caption{Experimental results comparing our approach against the baseline in the box environments (similar to those used during training) and in the photorealistic scenarios (Urban, Park and Office)}
% \resizebox{2\columnwidth}{!}{
% \label{tab:results}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% % \cline{2-19}
% \hline
% % \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% % {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% % {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
% \multirow{3}{*}{Method} & \multicolumn{16}{c|}{Experimental Scenarios and Metrics}\\
% \cline{2-17}
% & \multicolumn{4}{c|}{Box Environments} & \multicolumn{4}{c|}{Urban} & \multicolumn{4}{c|}{Park} & \multicolumn{4}{c|}{Office}\\
% \cline{2-17}
% & $P_{\theta}$ & $P_{\varphi}$ & $P_{\rho}$ & $P_{c}$ & $P_{\theta}$ & $P_{\varphi}$ & $P_{\rho}$ & $P_{c}$ & $P_{\theta}$ & $P_{\varphi}$ & $P_{\rho}$ & $P_{c}$ & $P_{\theta}$ & $P_{\varphi}$ & $P_{\rho}$ & $P_{c}$ \\
% \hline
% AOT \cite{zhao2021active} & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ \\
% \hline
% AD-VAT+ \cite{zhong2019ad} & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ & $ \cellcolor{red!30} 0.03$ \\
% \hline
% C-VAT \cite{devo2021enhancing} & $ \cellcolor{red!30} 0.05$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.05$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.05$ & $ \cellcolor{red!30} 0.04$  & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.05$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$ & $ \cellcolor{red!30} 0.04$\\
% \hline
% SiamRPN++ \cite{li2019siamrpn++} LQG & $ \cellcolor{yellow!40} 0.27$ & $ \cellcolor{yellow!40} 0.20$ & $ \cellcolor{yellow!40} 0.20$ & $ \cellcolor{yellow!40} 0.22$ & $ \cellcolor{yellow!40} 0.10$ & $ \cellcolor{yellow!40} 0.08$ & $ \cellcolor{yellow!40} 0.07$ & $ \cellcolor{yellow!40} 0.09$ & $ \cellcolor{yellow!40} 0.37$ & $ \cellcolor{yellow!40} 0.27$  & $ \cellcolor{yellow!40} 0.27$ & $ \cellcolor{yellow!40} 0.30$ & $ \cellcolor{yellow!40} 0.07$ & $ \cellcolor{yellow!40} 0.06$ & $ \cellcolor{yellow!40} 0.05$ & $ \cellcolor{yellow!40} 0.06$\\
% \hline
% SiamRPN++ \cite{li2019siamrpn++} PID & $ \cellcolor{yellow!40} 0.25$ & $ \cellcolor{yellow!40} 0.23$ & $ \cellcolor{yellow!40} 0.22$ & $ \cellcolor{yellow!40} 0.23$ & $ \cellcolor{yellow!40} 0.09$ & $ \cellcolor{yellow!40} 0.09$ & $ \cellcolor{yellow!40} 0.07$ & $ \cellcolor{yellow!40} 0.08$ & $ \cellcolor{yellow!40} 0.59$ & $ \cellcolor{yellow!40} 0.56$  & $ \cellcolor{yellow!40} 0.52$ & $ \cellcolor{yellow!40} 0.56$ & $ \cellcolor{yellow!40} 0.13$ & $ \cellcolor{yellow!40} 0.11$ & $ \cellcolor{yellow!40} 0.11$ & $ \cellcolor{yellow!40} 0.12$\\
% \hline
% D-VAT (Our) & $ \cellcolor{green!40} 0.94$ & $ \cellcolor{green!40} 0.94$ & $ \cellcolor{green!40} 0.86$ & $ \cellcolor{green!40} 0.91$ & $ \cellcolor{green!40} 0.94$ & $ \cellcolor{green!40} 0.94$ & $ \cellcolor{green!40} 0.91$ & $ \cellcolor{green!40} 0.93$ & $ \cellcolor{green!40} 0.95$ & $ \cellcolor{green!40} 0.95$  & $ \cellcolor{green!40} 0.92$ & $ \cellcolor{green!40} 0.94$ & $ \cellcolor{green!40} 0.95$ & $ \cellcolor{green!40} 0.95$ & $ \cellcolor{green!40} 0.86$ & $ \cellcolor{green!40} 0.92$\\
% \hline
% \end{tabular}}
% \vspace{-1em}
% \end{table*}

==> tables/tab_res_small.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Experimental results: positional tracking error in centimeters across different scenarios.}
\resizebox{0.48\textwidth}{!}{
\label{tab:results}
\begin{tabular}{|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{2}{*}{\shortstack{Observation\\Space}} & \multicolumn{4}{c|}{Experimental Scenarios}\\
\cline{2-5}
& Hover & Traj1 & Traj2 & Traj3\\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $\cellcolor{red!30} 4.6$ & $ \cellcolor{red!30} 5.7$ & $ \cellcolor{red!30} 6.8$ & $\cellcolor{red!30} 8.1$ \\
% \hline
% $\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $ \cellcolor{green!30} \textbf{2.7}$ & $ \cellcolor{green!30} \textbf{3.0}$ & $\cellcolor{green!30} \textbf{3.1}$ & $  \textbf{2.5}$ & $ 2.9 $ & $  6.2$ & $ \cellcolor{green!30} \textbf{3.9}$ \\
% \hline
% $\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  4.7 $ & $  3.0 $ & $  3.2 $ & $ \cellcolor{red!30} 3.7$ & $  6.7 $ & $  4.2 $ & $  4.4 $ & $ \cellcolor{red!30} 5.1$ & $  9.5 $ & $  3.1 $ & $  \textbf{3.1} $ & $ \cellcolor{red!30} 5.2$ & $  8.0 $ & $  2.9$ & $  6.6 $ & $ \cellcolor{red!30} 5.8$ \\
% \hline
% $\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  2.5 $ & $ 2.7 $ & $  3.1 $ & $ \cellcolor{green!30} \textbf{2.7}$ & $  4.0 $ & $  \textbf{3.3} $ & $ 3.6$ & $ \cellcolor{green!30} 3.6$ & $  4.1 $ & $3.0 $ & $  3.6 $ & $ \cellcolor{green!30} 3.5$ & $  3.1 $ & $  \textbf{2.6} $ & $ \textbf{5.8} $ & $ \cellcolor{green!30} \textbf{3.9}$ \\
% \hline
% $\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  \textbf{2.1} $ & $  3.2 $ & $  2.7 $ & $ \cellcolor{green!30} \textbf{2.7}$ & $  3.7 $ & $  5.0 $ & $  3.2$ & $ \cellcolor{yellow!30} 4.0$ & $  3.5$ & $  4.2 $  & $ 3.3 $ & $ \cellcolor{yellow!30} 3.6$ & $  4.2 $ & $  4.5 $ & $  \textbf{5.8} $ & $ \cellcolor{yellow!30} 4.8$\\
% \hline
% $\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$ & $ 2.2$ & $  3.7$ & $  3.1$ & $ \cellcolor{yellow!30} 3.0$ & $  3.2$ & $  4.7$ & $  3.0$ & $ \cellcolor{green!30} 3.6$ & $  3.3$ & $  4.2 $  & $  3.9 $ & $ \cellcolor{yellow!30} 3.8$ & $  3.5$ & $  4.3$ & $ 6.7$ & $ \cellcolor{yellow!30} 4.8$\\
% \hline
% \hline
% PID Controller & $ 1.6$ & $  1.5$ & $  1.4$ & $ \cellcolor{green!30} 1.5$ & $  2.4$ & $  5.5$ & $  1.6$ & $ \cellcolor{green!30} 3.2$ & $  2.8$ & $  2.7 $  & $  1.5 $ & $ \cellcolor{green!30} 2.3$ & $  3.4$ & $  2.6$ & $ 8.7$ & $ \cellcolor{yellow!30} 4.9$\\
\hline
\end{tabular}}
\vspace{-1.0em}
\end{table}

==> tables/tab_res_vel.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Positional tracking error in centimeters of the experiments conducted at increased speed.}
\resizebox{0.7\textwidth}{!}{
\label{tab:velresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{\shortstack{Observation\\Space\\Configuration}} & \multicolumn{12}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-13} & \multicolumn{4}{c|}{Planar Ellipse} & \multicolumn{4}{c|}{Planar Eight-Shape} & \multicolumn{4}{c|}{3D Eight-Shape}\\
\cline{2-13}
& $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  18.3$ & $  10.4$& $  3.5 $& $ \cellcolor{red!30} 10.7$& $  13.8 $& $  10.4 $& $  5.0 $& $ \cellcolor{red!30} 9.7$& $  15.0 $& $ 10.3$& $  6.9$& $ \cellcolor{red!30} 10.7$ \\
\hline
$\{ \mathbf{e}_\mathbf{w}, \mathbf{R},  \mathbf{u}\}$ & $  \textbf{3.6} $ & $  10.9 $& $  3.8 $& $ \cellcolor{green!30} \textbf{6.1}$& $ \textbf{4.0}$& $  \textbf{3.6} $& $  4.3 $& $ \cellcolor{green!30} \textbf{4.0}$& $  \textbf{3.8} $& $  \textbf{3.9} $& $  5.7$& $ \cellcolor{green!30} \textbf{4.5}$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R}, \mathbf{\omega},  \mathbf{u}\}$ & $  7.2 $ & $  15.6 $& $  9.2 $& $ \cellcolor{red!30} 10.7$& $  9.9 $& $  4.4 $& $  4.5$& $ \cellcolor{red!30} 6.3$& $  10.3$& $  4.7 $& $  7.5$& $ \cellcolor{red!30} 7.5$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{R},  \mathbf{u}\}$ & $  7.7 $ & $  11.8 $& $  7.0 $& $ \cellcolor{yellow!30} 8.8$& $  7.0 $& $  4.9$& $  4.2$& $ \cellcolor{yellow!30} 5.4$& $  8.5$& $  6.1 $& $  6.8 $& $ \cellcolor{yellow!30} 7.1$ \\
\hline
$\{ \mathbf{e}_\mathbf{b}, \mathbf{\omega},  \mathbf{u}\}$ & $  9.1 $ & $  \textbf{9.6} $& $  4.0 $& $ \cellcolor{yellow!30} 7.6$& $  4.4 $& $  5.7 $& $  \textbf{3.1} $& $ \cellcolor{green!30} 4.3$& $  5.5 $& $  6.4 $& $  5.9 $& $ \cellcolor{yellow!30} 5.9$ \\
\hline
$\{ \mathbf{e}_\mathbf{b},  \mathbf{u}\}$  & $  7.3 $ & $  10.1 $& $  \textbf{2.9} $& $ \cellcolor{green!30} 6.8$& $  7.0 $& $  7.2 $& $  3.3 $& $ \cellcolor{yellow!30} 5.9$& $  5.0 $& $  6.9 $& $  \textbf{4.7} $& $ \cellcolor{green!30} 5.5$ \\
\hline
\hline
PID Controller  & $  7.8 $ & $  15.6 $& $  2.2 $& $ \cellcolor{yellow!30} 8.5$& $  7.9 $& $  5.8 $& $  1.5 $& $ \cellcolor{yellow!30} 5.1$& $  8.2 $& $  5.8 $& $  16.8 $& $ \cellcolor{red!30} 10.3$ \\
\hline
\end{tabular}}
\vspace{-1.0em}
\end{table*}

==> tables/tab_res_vel_backup.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\centering
\caption{Max Velocity: experimental results. We report the mean over 3 runs of the x y z error RMSE and (peak) values.}
\resizebox{\textwidth}{!}{
\label{tab:velresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \cline{2-19}
\hline
% \multirow{3}{*}{\backslashbox{Method}{Scenario}}
% {\backslashbox{Sequence}{Metric}} & $SR$ & $S\text{-}DOD$ & $CE$ & $SR$ & $S\text{-}DOD$ & $CE$ \\
% {\backslashbox{Delay ($\delta$)}{Mass coeff. ($\alpha$)}} & 0.6 & 0.7 & 0.8 & 0.9 & 1.0 & 1.1 & 1.2 & 1.3 & 1.4 &\\
\multirow{3}{*}{Input Type} & \multicolumn{12}{c|}{Experimental Scenarios and Metrics}\\
\cline{2-13} & \multicolumn{4}{c|}{Oval Trajectory} & \multicolumn{4}{c|}{Otto Trajectory} & \multicolumn{4}{c|}{Special Trajectory}\\
\cline{2-13}
& $P_{x}$ & $P_{y}$ & $P_{z}$ & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ & $P_{x}$ & $P_{y}$ & $P_{z}$  & $P_{c}$ \\
\hline
pRwa World & $ \cellcolor{red!30} 18.3 \,(35.2)$ & $ \cellcolor{yellow!30} 10.4 \,(22.1)$& $ \cellcolor{green!30} 3.5 \,(8.5)$& $ \cellcolor{red!30} 10.7$& $ \cellcolor{red!30} 13.8 \,(27.4)$& $ \cellcolor{red!30} 10.4 \,(20.7)$& $ \cellcolor{red!30} 5.0 \,(10.4)$& $ \cellcolor{red!30} 9.7$& $ \cellcolor{red!30} 15.0 \,(29.1)$& $ \cellcolor{red!30} 10.3 \,(19.1)$& $ \cellcolor{red!30} 6.9 \,(13.9)$& $ \cellcolor{red!30} 10.7$ \\
\hline
pRa World & $ \cellcolor{green!30} \textbf{3.6} \,(\textbf{9.2})$ & $ \cellcolor{yellow!30} 10.9 \,(18.6)$& $ \cellcolor{yellow!30} 3.8 \,(9.0)$& $ \cellcolor{green!30} \textbf{6.1}$& $ \cellcolor{green!30} \textbf{4.0} \,(\textbf{9.6})$& $ \cellcolor{green!30} \textbf{3.6} \,(\textbf{9.2})$& $ \cellcolor{yellow!30} 4.3 \,(9.9)$& $ \cellcolor{green!30} \textbf{4.0}$& $ \cellcolor{green!30} \textbf{3.8} \,(\textbf{7.9})$& $ \cellcolor{green!30} \textbf{3.9} \,(\textbf{10.0})$& $ \cellcolor{yellow!30} 5.7 \,(13.0)$& $ \cellcolor{green!30} \textbf{4.5}$ \\
\hline
pRwa Body & $ \cellcolor{yellow!30} 7.2 \,(16.5)$ & $ \cellcolor{red!30} 15.6 \,(28.6)$& $ \cellcolor{red!30} 9.2 \,(20.1)$& $ \cellcolor{red!30} 10.7$& $ \cellcolor{red!30} 9.9 \,(20.6)$& $ \cellcolor{green!30} 4.4 \,(10.7)$& $ \cellcolor{red!30} 4.5 \,(10.4)$& $ \cellcolor{red!30} 6.3$& $ \cellcolor{red!30} 10.3 \,(22.1)$& $ \cellcolor{red!30} 4.7 \,(10.9)$& $ \cellcolor{red!30} 7.5 \,(17.0)$& $ \cellcolor{red!30} 7.5$ \\
\hline
pRa Body & $ \cellcolor{yellow!30} 7.7 \,(16.8)$ & $ \cellcolor{red!30} 11.8 \,(22.1)$& $ \cellcolor{red!30} 7.0 \,(17.5)$& $ \cellcolor{yellow!30} 8.8$& $ \cellcolor{yellow!30} 7.0 \,(14.5)$& $ \cellcolor{yellow!30} 4.9 \,(11.5)$& $ \cellcolor{yellow!30} 4.2 \,(11.9)$& $ \cellcolor{yellow!30} 5.4$& $ \cellcolor{yellow!30} 8.5 \,(18.4)$& $ \cellcolor{yellow!30} 6.1 \,(17.1)$& $ \cellcolor{yellow!30} 6.8 \,(15.5)$& $ \cellcolor{yellow!30} 7.1$ \\
\hline
pwa Body & $ \cellcolor{red!30} 9.1 \,(19.5)$ & $ \cellcolor{green!30} \textbf{9.6} \,(19.8)$& $ \cellcolor{yellow!30} 4.0 \,(10.7)$& $ \cellcolor{yellow!30} 7.6$& $ \cellcolor{green!30} 4.4 \,(10.7)$& $ \cellcolor{yellow!30} 5.7 \,(12.5)$& $ \cellcolor{green!30} \textbf{3.1} \,(8.3)$& $ \cellcolor{green!30} 4.3$& $ \cellcolor{yellow!30} 5.5 \,(12.0)$& $ \cellcolor{yellow!30} 6.4 \,(13.7)$& $ \cellcolor{green!30} 5.9 \,(13.4)$& $ \cellcolor{yellow!30} 5.9$ \\
\hline
pa Body & $ \cellcolor{yellow!30} 7.3 \,(17.0)$ & $ \cellcolor{green!30} 10.1 \,(\textbf{19.0})$& $ \cellcolor{green!30} \textbf{2.9} \,(\textbf{7.2})$& $ \cellcolor{yellow!30} 6.8$& $ \cellcolor{red!30} 7.0 \,(16.9)$& $ \cellcolor{red!30} 7.2 \,(14.2)$& $ \cellcolor{green!30} 3.3 \,(\textbf{8.2})$& $ \cellcolor{yellow!30} 5.9$& $ \cellcolor{green!30} 5.0 \,(11.4)$& $ \cellcolor{yellow!30} 6.9 \,(14.7)$& $ \cellcolor{green!30} \textbf{4.7} \,(\textbf{11.9})$& $ \cellcolor{green!30} 5.5$ \\
\hline
\end{tabular}}
\vspace{-0.8em}
\end{table*}

==> tables/variables.tex <==
\begin{table}[h]
% \vspace{-0.5em}
\centering
%\caption{Notation: vectors, matrices and and scalars with the corresponding dimension.}
\resizebox{\columnwidth}{!}{
\label{tab:notation}
\begin{tabular}{cccccccccc}
\hline
\Tstrut \Bstrut
\textbf{Mat - Vec} & $x$& $p$& $v$& $R$& $\omega$& $\omega_{cmd}$ & $J$& $f_{drag}$& $g$ \\
\hline
\textbf{Dimension} & $19\times1$& $3\times1$& $3\times1$& $3\times3$& $3\times1$& $3\times1$& $3\times3$& $3\times1$& $3\times1$ \Tstrut\Bstrut\\ 
\hline
\hline
\Tstrut \Bstrut
\textbf{Scalars} & $m$& $f$& $f_{cmd}$& $k_f$& $k_{\omega}$& $k_{vx}$& $k_{vy}$& $k_{vz}$& \Tstrut\Bstrut\\ 
\hline
\end{tabular}}
% \vspace{-1.2em}
\end{table}

\begin{comment}
\begin{table*}[t]
% \vspace{-0.5em}
\centering
%\caption{Notation: vectors, matrices and and scalars with the corresponding dimension.}
\resizebox{\textwidth}{!}{
\label{tab:notation}
\begin{tabular}{cccccccccccccccccc}
\hline
\Tstrut \Bstrut
\textbf{Symbol} & $x$& $p$& $v$& $R$& $\omega$& $\omega_{cmd}$ & $m$& $J$& $f$& $f_{cmd}$& $f_{drag}$& $g$& $k_f$& $k_{\omega}$& $k_{vx}$& $k_{vy}$& $k_{vz}$ \\
\hline
\textbf{Dimension} & $19\times1$& $3\times1$& $3\times1$& $3\times3$& $3\times1$& $3\times1$& $1$& $3\times3$& $1$& $1$& $3\times1$& $3\times1$& 1& 1& 1& 1& 1 \Tstrut\Bstrut\\ 
\hline
\end{tabular}}
% \vspace{-1.2em}
\end{table*}
\end{comment}
